Causality matters in medical imaging

This article discusses how the language of causality can shed new light on the major challenges in machine learning for medical imaging: 1) data scarcity, which is the limited availability of high-quality annotations, and 2) data mismatch, whereby a trained algorithm may fail to generalize in clinical practice. Looking at these challenges through the lens of causality allows decisions about data collection, annotation procedures, and learning strategies to be made (and scrutinized) more transparently. We discuss how causal relationships between images and annotations can not only have profound effects on the performance of predictive models, but may even dictate which learning strategies should be considered in the first place. For example, we conclude that semi-supervision may be unsuitable for image segmentation---one of the possibly surprising insights from our causal analysis, which is illustrated with representative real-world examples of computer-aided diagnosis (skin lesion classification in dermatology) and radiotherapy (automated contouring of tumours). We highlight that being aware of and accounting for the causal relationships in medical imaging data is important for the safe development of machine learning and essential for regulation and responsible reporting. To facilitate this we provide step-by-step recommendations for future studies.

==> fig/dataset_shift_offset.tex <==
{
\tikzset{x=1cm, y=.5cm}
\renewcommand{\given}{\vert}
\renewcommand{\Prob}[2][]{P_{#1}(#2)}
\begin{subfigure}{.32\textwidth}
    \centering
    \begin{tikzpicture}
        \node[unobs,label={left:$Z$}]   at (0,0) (z) {};
        \node[obs,  label={90:$X$}]     at (1,0) (x) {};
        \node[obs,  label={right:$Y$}]  at (2,0) (y) {};
        % \node[dom,  label={$D$}]        at (0,1) (d) {};
        \path (0,1) node[dom] (d) {} ++(160:8pt) node {$D$};
        \draw (z) edge (x);
        \draw (x) edge (y);
        \draw (d) edge (z);
    \end{tikzpicture}
    \caption{\centering Population shift: ${\boldsymbol{\Prob[D]{Z}}\Prob{X\given Z}\Prob{Y\given X}}$}
    \label{fig:covariate_shift}
\end{subfigure} \hfill
\begin{subfigure}{.34\textwidth}
    \centering
    \begin{tikzpicture}
        \node[unobs,label={left:$Z$}]   at (0,0) (z) {};
        \node[obs,  label={45:$X$}]     at (1,0) (x) {};
        \node[obs,  label={right:$Y$}]  at (2,0) (y) {};
        % \node[dom,  label={$D$}]        at (1,1) (d) {};
        \path (1,1) node[dom] (d) {} ++(160:8pt) node {$D$};
        \draw (z) edge (x);
        \draw (x) edge (y);
        \draw (d) edge (x);
    \end{tikzpicture}
    \caption{\centering Causal acquisition shift: ${\Prob{Z}\boldsymbol{\Prob[D]{X\given Z}}\Prob{Y\given X}}$}
    \label{fig:concept_shift}
\end{subfigure} \hfill
\begin{subfigure}{.32\textwidth}
    \centering
    \begin{tikzpicture}
        \node[unobs,label={left:$Z$}]   at (0,0) (z) {};
        \node[obs,  label={90:$X$}]     at (1,0) (x) {};
        \node[obs,  label={right:$Y$}]  at (2,0) (y) {};
        % \node[dom,  label={$D$}]        at (2,1) (d) {};
        \path (2,1) node[dom] (d) {} ++(160:8pt) node {$D$};
        \draw (z) edge (x);
        \draw (x) edge (y);
        \draw (d) edge (y);
    \end{tikzpicture}
    \caption{\centering Annotation shift: ${\Prob{Z}\Prob{X\given Z}\boldsymbol{\Prob[D]{Y\given X}}}$}
    \label{fig:conditional_shift}
\end{subfigure} \\[1ex]
\begin{subfigure}{.32\textwidth}
    \centering
    \begin{tikzpicture}
        \node[obs,  label={left:$X$}]   at (0,0) (x) {};
        \node[unobs,label={90:$Z$}]     at (1,0) (z) {};
        \node[obs,  label={right:$Y$}]  at (2,0) (y) {};
        % \node[dom,  label={$D$}]        at (2,1) (d) {};
        \path (2,1) node[dom] (d) {} ++(10:7pt) node {$D$};
        \draw (y) edge (z);
        \draw (z) edge (x);
        \draw (d) edge (y);
    \end{tikzpicture}
    \caption{\centering Prevalence shift: ${\Prob{X\given Z}\Prob{Z\given Y}\boldsymbol{\Prob[D]{Y}}}$}
    \label{fig:target_shift}
\end{subfigure} \hfill
\begin{subfigure}{.32\textwidth}
    \centering
    \begin{tikzpicture}
        \node[obs,  label={left:$X$}]   at (0,0) (x) {};
        \node[unobs,label={135:$Z$}]    at (1,0) (z) {};
        \node[obs,  label={right:$Y$}]  at (2,0) (y) {};
        % \node[dom,  label={$D$}]        at (1,1) (d) {};
        \path (1,1) node[dom] (d) {} ++(10:7pt) node {$D$};
        \draw (y) edge (z);
        \draw (z) edge (x);
        \draw (d) edge (z);
    \end{tikzpicture}
    \caption{\centering Manifestation shift: ${\Prob{X\given Z}\boldsymbol{\Prob[D]{Z\given Y}}\Prob{Y}}$}
\end{subfigure} \hfill
\begin{subfigure}{.32\textwidth}
    \centering
    \begin{tikzpicture}
        \node[obs,  label={left:$X$}]   at (0,0) (x) {};
        \node[unobs,label={90:$Z$}]     at (1,0) (z) {};
        \node[obs,  label={right:$Y$}]  at (2,0) (y) {};
        % \node[dom,  label={$D$}]        at (0,1) (d) {};
        \path (0,1) node[dom] (d) {} ++(10:7pt) node {$D$};
        \draw (y) edge (z);
        \draw (z) edge (x);
        \draw (d) edge (x);
    \end{tikzpicture}
    \caption{\centering Anticausal acqn.\ shift: ${\boldsymbol{\Prob[D]{X\given Z}}\Prob{Z\given Y}\Prob{Y}}$}
\end{subfigure}
}

\caption{Selection diagrams for (a--c) causal (d--f) and anticausal dataset shift scenarios, with corresponding factorizations of the joint $\Prob[D]{X,Y,Z}$. $X$ denotes the acquired image, $Y$ is the prediction target, $Z$ is the subject's unobserved true anatomy, and $D$ is the domain indicator ($0=$ `train', $1=$ `test').}


==> fig/dataset_shift_old.tex <==
\tikzset{x=.75cm, y=.5cm}
\begin{subfigure}{.23\textwidth}
    \centering
    \begin{tikzpicture}
        \node[obs, label={left:$X$}]    at (0,0) (x) {};
        \node[obs, label={right:$Y$}]   at (2,0) (y) {};
        \node[dom, label={$D$}]         at (1,1) (d) {};
        \draw (x) edge (y);
        \draw (d) edge (x);
    \end{tikzpicture}
    \caption{\centering Covariate shift: $\Prob{X \given D} \Prob{Y \given X}$}
    \label{fig:covariate_shift}
\end{subfigure} \hfill
\begin{subfigure}{.23\textwidth}
    \centering
    \begin{tikzpicture}
        \node[obs, label={left:$X$}]    at (0,0) (x) {};
        \node[obs, label={right:$Y$}]   at (2,0) (y) {};
        \node[dom, label={$D$}]         at (1,1) (d) {};
        \draw (x) edge (y);
        \draw (d) edge (y);
    \end{tikzpicture}
    \caption{\centering Concept shift: $\Prob{X} \Prob{Y \given X,D}$}
    \label{fig:concept_shift}
\end{subfigure} \hfill
\begin{subfigure}{.23\textwidth}
    \centering
    \begin{tikzpicture}
        \node[obs, label={left:$X$}]    at (0,0) (x) {};
        \node[obs, label={right:$Y$}]   at (2,0) (y) {};
        \node[dom, label={$D$}]         at (1,1) (d) {};
        \draw (y) edge (x);
        \draw (d) edge (y);
    \end{tikzpicture}
    \caption{\centering Target shift: $\Prob{X \given Y} \Prob{Y \given D}$}
    \label{fig:target_shift}
\end{subfigure} \hfill
\begin{subfigure}{.25\textwidth}
    \centering
    \begin{tikzpicture}
        \node[obs, label={left:$X$}]    at (0,0) (x) {};
        \node[obs, label={right:$Y$}]   at (2,0) (y) {};
        \node[dom, label={$D$}]         at (1,1) (d) {};
        \draw (y) edge (x);
        \draw (d) edge (x);
    \end{tikzpicture}
    \caption{\centering Conditional shift: $\Prob{X \given Y,D} \Prob{Y}$}
    \label{fig:conditional_shift}
\end{subfigure} \\[1ex]
\begin{subfigure}{.29\textwidth}
    \centering
    \optional{
    \begin{tikzpicture}
        \node[obs,  label={left:$X$}]   at (0,0) (x) {};
        \node[unobs,label={$X_0$}]      at (1,1) (x0){};
        \node[obs,  label={right:$Y$}]  at (2,0) (y) {};
        \node[dom,  label={$D$}]        at (0,1) (d) {};
        \draw (x0) edge (x);
        \draw (x) edge (y);
        \draw (d) edge (x);
    \end{tikzpicture}
    \caption{\centering Causal domain shift%: $\sum_{x_0} \big[\mathopen{}\Prob{X \given x_0, D} \Prob{x_0,Y}\big]$}
    }}
\end{subfigure} \hfill
\begin{subfigure}{.34\textwidth}
    \centering
    \optional{
    \begin{tikzpicture}
        \node[obs,  label={left:$X$}]   at (0,0) (x) {};
        \node[unobs,label={$X_0$}]      at (1,1) (x0){};
        \node[obs,  label={right:$Y$}]  at (2,0) (y) {};
        \node[dom,  label={$D$}]        at (0,1) (d) {};
        \draw (x0) edge (x);
        \draw (y) edge (x0);
        \draw (d) edge (x);
    \end{tikzpicture}
    \caption{\centering Anticausal domain shift%: $\big[\sum_{x_0} \Prob{X \given x_0, D} \Prob{x_0}\big] \Prob{Y \given X}$}
    }}
\end{subfigure} \hfill
\begin{subfigure}{.35\textwidth}
    \centering
    \optional{
    \begin{tikzpicture}
        \node[obs,  label={left:$X$}]   at (0,0) (x) {};
        \node[unobs,label={$X_0$}]      at (1,1) (x0){};
        \node[obs,  label={right:$Y$}]  at (2,0) (y) {};
        \node[dom,  label={$D$}]        at (0,1) (d) {};
        \draw (x0) edge (x) edge (y);
        \draw (d) edge (x);
    \end{tikzpicture}
    \caption{\centering Confounded domain shift%: $\big[\sum_{x_0} \Prob{X \given x_0} \Prob{x_0 \given D}\big] \Prob{Y \given X}$}
    }}
\end{subfigure}
% \begin{subfigure}{.48\textwidth}
%     \centering
%     \optional{
%     \begin{tikzpicture}[x=2cm, y=1.5cm]
%         \node[obs,  label={left:$X$}]   at (0,0)    (x) {};
%         \node[unobs,label={above:$X_0$}]at (.5,.5)  (x0){};
%         \node[obs,  label={right:$Y$}]  at (1,0)    (y) {};
%         \node[dom,  label={$D$}]        at (0,.5)   (d) {};
%         \draw (x0) edge (x);
%         \draw (d) edge (x);
%         \draw[optional] (x) edge (y) (x0) edge[bend left=15] (y) (y) edge[bend left=15] (x0);
%     \end{tikzpicture}
%     \caption{\centering Domain shift: ${\big[\sum_{x_0} \Prob{X \given x_0, D} \Prob{x_0}\big] \Prob{Y \given X}}$}
%     }
% \end{subfigure}

\caption{Selection diagrams for canonical dataset shift scenarios, with the corresponding factorization of the joint $\Prob{X,Y \given D}$. $X$ denotes features, $Y$ is the prediction target, and $D$ is the domain indicator ($0=$ `train', $1=$ `test'). \optional{\mbox{(e--g)}~Types of domain shift. $X_0$ is the subject's unobserved true anatomy.}}


==> tikzlibrarycausal.code.tex <==
\usetikzlibrary{arrows.meta, decorations.pathmorphing}

% Causal diagram style macros
\tikzset{x=.75cm, y=.75cm}

\tikzset{font=\sffamily\footnotesize}

% Edge styles
\tikzset{>={Triangle[length=6pt, width=3pt]}}
\tikzset{every edge/.append style={->}}
\tikzstyle{confounded} = [<->, densely dashed, bend right]
\tikzstyle{undir} = [-]
\tikzstyle{optional} = [->, densely dotted, gray]
% \tikzstyle{proxy} = [double, double distance=1pt]
\tikzstyle{proxy} = [->, decorate, decoration={snake, post length=6pt, segment length=5pt, amplitude=.8pt}]
% Node styles
\tikzset{every label/.append style={inner sep=0pt, label distance=3pt}}
\tikzstyle{obs} = [draw, fill, circle, inner sep=0pt, minimum size=4pt]
\tikzstyle{unobs} = [obs, fill=none]
\tikzstyle{dom} = [obs, rectangle, minimum size=3.5pt]
\tikzstyle{sel} = [unobs, minimum size=6pt, append after command={
    \pgfextra{\node[unobs, minimum size=3pt] at (\tikzlastnode) {};}}]

% Connect all nodes #2 to all nodes #3. Borrowed from: 
% https://github.com/jluttine/tikz-bayesnet/blob/master/tikzlibrarybayesnet.code.tex
\newcommand{\edge}[3][]{%
    \foreach \x in {#2} {%
        \foreach \y in {#3} {%
            \path (\x) edge[#1] (\y);%
        };%
    };%
}

\newcommand{\chain}[2][]{
    \foreach \y [count=\i, remember=\y as \x] in {#2} {%
        \ifnum\i>1%
            \path (\x) edge[#1] (\y);%
        \fi%
    };%
}

